The Shapley Taylor Interaction Index

The attribution problem, that is the problem of attributing a model's prediction to its base features, is well-studied. We extend the notion of attribution to also apply to feature interactions. The Shapley value is a commonly used method to attribute a model's prediction to its base features. We propose a generalization of the Shapley value called Shapley-Taylor index that attributes the model's prediction to interactions of subsets of features up to some size k. The method is analogous to how the truncated Taylor Series decomposes the function value at a certain point using its derivatives at a different point. In fact, we show that the Shapley Taylor index is equal to the Taylor Series of the multilinear extension of the set-theoretic behavior of the model. We axiomatize this method using the standard Shapley axioms -- linearity, dummy, symmetry and efficiency -- and an additional axiom that we call the interaction distribution axiom. This new axiom explicitly characterizes how interactions are distributed for a class of functions that model pure interaction. We contrast the Shapley-Taylor index against the previously proposed Shapley Interaction index (cf. [9]) from the cooperative game theory literature. We also apply the Shapley Taylor index to three models and identify interesting qualitative insights.

==> computation.tex <==
\section{Computation}

\subsection{Approximation through sampling}
The exact computation of \prefixvalues can be done using the formulas from Section~\ref{sec:method}.
Both methods require exponential running time.


Using sampling method, we can construct a FPRAS~\footnote{verify this} to
estimate \prefixvalues. The sampling algorithm is as follows:
\begin{enumerate}
  \item Generate $k$ permutations randomly. Compute the expected value over these $k$ permutations as in Equation~\ref{eq:randorder}.
  \item Repeat step $m$ times and compute the median of the $m$ estimates.
\end{enumerate}


\begin{theorem}
  For $k = O(\frac{u^2}{\epsilon^2})$ and $m = \log(\frac{1}{\delta})$, the
  algorithm has error $\leq \epsilon$ with probability $\geq 1-\delta$.
\end{theorem}

\subsection{Special cases}
For functions computed by decision trees, we can use Algorithm 2
of~\cite{Lundberg18} with little modifications.


==> deleted.tex <==
\subsection{The Roles of the Axioms}
\label{sec:ax-discussion}

Here we discuss informally the roles that the various axioms play, and specifically, the need for the interaction distribution axiom. For simplicity, we consider explanations of order $k=2$. Consider the space of interaction distribution methods that satisfy linearity. It is well-known that the set of unanimity \games (defined as $\V_T(S) = 1$ if $T \subseteq S$ and $0$ otherwise) constitute a basis for the space of all \games. 
%That is, every \game $v$, can be expressed as a unique linear combination of these \games. By linearity, the interaction
%indices for the \game $v$ should be the same linear combination of the interaction indices for the unanimity \games. 
Therefore, defining the interaction indices for unanimity \games specifies the interaction indices for all \games.

Specifically, consider the unanimity \game defined for a set $T \subseteq N$ , such that $|T| >1$. 
%Now let us consider the effect of the Dummy and Symmetry axioms. 
Dummy axiom constrains us from attributing to interaction terms that contain elements not in $T$.  Symmetry dictates that all the main effects for \players in $T$ are same (say $a_T$), and all the pairs $(i,j)$ such that $i \in $ and $j \in T$, get the same interaction effect (say $b_T$). 

Recall that \siv satisfy Linearity, Dummy and Symmetry, and as we show later, so do \stv. Pairwise \siv assign a value of $b_T = 1/(|T|-1)$ to every one of the ${|T| \choose 2}$ pairs of elements. Pairwise \siv does not define main effect terms, but for simplicity, we can consider $a_T =0$. Pairwise \siv thus violate efficiency. 

\stv assign a value of $b_T = 1/{|T| \choose  2}$ to every pair of elements from the set $T$ and $a_T= 0$; this satisfies symmetry, dummy, linearity, but also efficiency. However, this is not the unique way to satisfy efficiency; there are other assignments to $a_T$ and $b_T$ that still satisfy efficiency. \footnote{A different method is to apply the Shapley value to the Shapley value; i.e. treat the Shapley value of an element itself as a set function and apply Shapley value on that set function. It turns out that this is well-defined. Doing so sets $a_T = b_T$. While it is an open question to identify an axiom that causes this assignment,  this does show that the approach of explicitly defining interactions for interaction \games (recall that every basis function is an interaction \games) is interesting beyond \stv.} This ambiguity is tied to non-orthogonality----the singleton sets are not orthogonal to the pairs. As a consequence, we need an additional axiom to pin down the interaction index. In our case, the interaction distribution axiom causes the explicit choice of setting the main effect terms $a_T$ to zero. This prevents the main effect of individual \players from getting credit from higher order interactions (recall that we are discussing the case $|T| >1$). 

In contrast, notice that the assignment to the pairwise \shares is reductive---the
pairwise \shares capture not only the pairwise interactions ($|T|=2$) , but also larger interactions ($|T|>2$). This reductiveness is necessitated by
the constraint on the order of explanation ($k=2$) and the efficiency axiom. Notice that the very same reductiveness is present in the Shapley value (order of explanation $k=1$); recall that the Shapley value is the \stv when $k=1$, see Section~\ref{sec:taylor}. In the Shapley value, all the interactions are redistributed among the main effects. As we increase the order of explanation, the amount of reductiveness decreases---progressively larger interactions (of size $k-1$ or less) are captured unambiguously. However, this is at the cost of more computation and a longer explanation.



\section{Other deleted material}

\begin{proposition}\label{prop:completeness}
The \prefixvalues satisfy the completeness axiom. Formally:
$$v(N) - v(\emptyset) = \sum_i \interaction_i(v) + \sum_{i, j} \interaction_{ij}(v)$$
\end{proposition}

\begin{proof}
We'll prove completeness of $\interaction_{ij, \pi}$ for each permutation $\pi$.
Without loss of generality, consider the permutation $\pi = [1, 2, \ldots, n]$. Recall that $\pi^i = \{1, \ldots, i \}$ denote the predecessors of $i$ in permutation $\pi$.

We'll use induction to prove the following statement:
$$ \sum_{i, j \leq k} \interaction_{ij, \pi}(v) + \sum_{i \leq k} \phi_i(v) = v(\pi^k) - v(\emptyset)$$

The base case of induction is $k = 1$. LHS is $\phi_1(v) = \delta_1(\emptyset) = v(\pi^1) - v(\emptyset)$. This 
proves the base case. 

For the induction step, we'll assume the equation to be true for $k-1$ and prove it for $k$.

\begin{align*}
    LHS & = \sum_{i, j \leq k} \interaction_{ij, \pi}(v) + \sum_{i \leq k} \interaction_i(v) \\
    & = \sum_{i, j \leq k-1} \interaction_{ij, \pi}(v) + \sum_{i \leq k-1} \interaction_i(v) + \sum_{i < k} \interaction_{ik, \pi}(v) + \interaction_k(v) \\
    & = v(P_{k-1}) - v(\emptyset) + \sum_{i < k} \interaction_{ik, \pi}(v) + \interaction_k(v) \\
\end{align*}

We simplify the equation by examining the last two terms:
\begin{align*}
    \sum_{i < k} \interaction_{ik, \pi}(v) + \interaction_k(v) & =  \sum_{i < k} (v(\pi^i \cup \{ k \})  - v(\pi^{i-1} \cup \{ k \}) - v(\pi^i) + v(\pi^{i-1})) + v(\{k\}) - v(\emptyset)\\
    & =  v(\pi^k) - v(\{ k \}) - v(\pi^{k-1}) + v(\emptyset) + v(\{k\}) - v(\emptyset)\\
    & = v(\pi^k) - v(\pi^{k-1}) \\
\end{align*}

Substituting back in the above equation:
\begin{align*}
    LHS & = v(\pi^{k-1}) - v(\emptyset) + v(\pi^k) - v(\pi^{k-1}) \\
    & = v(\pi^k) - v(\emptyset) \\
\end{align*}
This proves the inductive step. The completeness for expectation over all permutations follows from the linearity of expectations.
\end{proof}


\subsection*{Uniqueness}
In this section, we prove that \prefixvalues are the only interaction indices that satisfy all the axioms.

We start our derivation by considering unanimity games $u_T$ defined as: $u_T(S) = 1$ if $T \subseteq S$ and $0$ otherwise. Let $\phi$ be an interaction index that satisfies axioms 1-5.

Dummy axiom implies that $\phi_{i}(u_T) = 0$ for $i \not\in T$. Moreover,
if $i \not\in T$ or $j \not\in T$, then we also have $\phi_{ij}(u_T) = 0$.\footnote{Check this again.}

Total contribution from individual and pairwise values in $T$ can be written as:

\begin{equation}\label{eq:completeness}
u_T(N) = \sum_{i \in T} \phi_i(u_T) + \sum_{i, j \in T} \phi_{ij}(u_T)    
\end{equation}

Now, using the efficiency axiom, we get:
\begin{equation}\label{eq:complete_inter}
\sum_{i \in T} \phi_i(u_T) + \sum_{i, j \in T} \phi_{ij}(u_T) = 1
\end{equation}



\subsection{Interaction distribution axiom and the Shapley Interaction index}
\todo{What purpose does this subsection have? How does it make the paper stronger? Delete?}
We compare the \prefixvalues with Shapley interaction index on unanimity games.
We start with Shapley interaction index defined Equation (5) of~\cite{Grabisch99}:

\begin{align*}
I(ij, V_T) & = \frac{1}{n-1} \sum_{S \subseteq N \setminus \{i,j\} } \frac{1}{{n-2 \choose s}} \delta_{ij}(S) \\
& = \frac{1}{n-1} \sum_{S \subseteq N \setminus \{i,j\} } \frac{1}{{n-2 \choose s}} (v_T(S \cup \{i, j\}) - v_T(S \cup \{ i \}) - v_T(S \cup \{ j \}) + v_T(S))
\end{align*}

At this point, we inspect two cases separately. First one is where $i \not\in T$. In this case, $v_T(S \cup \{i, j\}) = v_T(S \cup \{ j\})$ and $v_T(S \cup \{ j \}) = v_T(S)$. Therefore, $\delta_{ij}(S) = 0$. Similar argument applies to
the case where $j \not\in T$.

Now, consider the case where $i, j \in T$. In this case $v_T(S \cup \{i, j\}) = 1$ if $S \supseteq T$, but the
other terms in the summation are $0$, as $i, j \not\in S$, hence $T \not\subseteq S \cup \{ i \}$ and $T \not\subseteq S \cup \{ j \}$. This gives us the following:

\begin{align*}
I(ij, V_T) & = \frac{1}{n-1} \sum_{S \subseteq N \setminus \{i,j\}, S \supseteq T} \frac{1}{{n-2 \choose s}} \\
& = \frac{1}{n-1} \sum_{s = t-2}^{n-2} \frac{{n-t \choose t-a+2}}{{n-2 \choose s}} \\
& = \frac{1}{n-1} \sum_{s = t-2}^{n-2} \frac{{s \choose t-2}}{{n-2 \choose t-2}} \\
& = \frac{1}{n-1} \frac{{n-1 \choose t-1}}{{n-2 \choose t-2}} \\
& = \frac{1}{t-1} \\
\end{align*}
Contrast this with \prefixvalues on unanimity games, where each $\interaction_{ij}$ is $\frac{1}{t(t-1)}$.







We start with the second order Taylor expansion with Lagrange remainder:
$$ g(1) - g(0) = g'(0) + \int_{t=0}^1 (1-t) g''(t) dt $$

We show that the two terms on the right side of this equation correspond to the \prefixvalues for singletons and pairs respectively. 

Here $g(1) = f(1, \ldots, 1) = v(N)$ and $g(0) = f(0, \ldots, 0) = v(\emptyset)$.
\begin{claim}
$g'(0) = \sum_i \phi_i(v)$
\end{claim}
\begin{proof}
Let $f_i$ denote the partial derivative with respect to $x_i$, i.e. $f_i = \frac{\partial f}{\partial x_i}$.
By chain rule, we have $g'(0) = \sum_i f_i(0)$.
Owen~\cite{Owen72} showed that $$f_i(x) = \sum_{S \subseteq N \setminus \{ i \}} \prod_{j \in S} x_j \prod_{j \not\in S, j \neq i} (1 - x_j) \delta_i(S)$$
Hence $f_i(0, \ldots, 0) = \delta_i(\emptyset)$, which is same as $\phi_i(v)$. This proves the claim.
\end{proof}

\begin{claim}
$\int_{t=0}^1 (1-t) f''(t) dt = \sum_{i, j} \phi_{ij}(v)$
\end{claim}
\begin{proof}
Let $f_{ij}(t)$ denote the second partial derivative with respect to $i$ and $j$. By chain rule, we have 
$$ f''(t) = \sum_{i, j} f_{ij}(t)$$

For each $f_{ij}(t)$, we can write them as follows:
%\footnote{This is similar to Owen's calculation~\cite{Owen72}.}

\begin{align*}
f_{ij}(t) & = \sum_{S \subseteq N \setminus \{i,j\}} \prod_{a \in S} x_a \prod_{a \not\in S \cup \{i, j\} } (1-x_a) \cdot \delta_{ij}(S) \\
\end{align*}

$$f_{ij}(t) = \sum_{S \subseteq N \setminus \{i,j\}} \delta_{ij}(S) t^s (1-t)^{n-s-2} $$
Hence, we get
\begin{align*}
\int_0^1 (1-t) f_{ij}(t) dt & = \sum_{S \subseteq N \setminus \{i,j\}} \delta_{ij}(S) \int_0^1 t^s (1-t)^{n-s-1} dt \\ 
& = \frac{1}{n} \sum_{S \subseteq N \setminus \{i,j\}} \delta_{ij}(S) / {n-1 \choose s}
\end{align*}


\end{proof}






\subsubsection*{Proof of Proposition~\ref{prop:efficiency}}



\begin{proof}


Consider a permutation $\pi$ and consider $\interaction_{S, \pi}(v)$ defined by Equation~\ref{eq:permutation}. For sets $S$
such that $|S| < k$, we have $\interaction_{S, \pi}(v) = \delta_{S} v(\emptyset)$. We define the sum of all the \prefixvalues
for a fixed size $j$ ($j < k$) as follows:

\begin{align}
M^k_j & := \sum_{|S| = j} \interaction_{S, \pi}(v) \notag \\
& = \sum_{|S| = j} \delta_{S} v(\emptyset)  \\
& = \sum_{\{i_1 < \ldots < i_j \}} \delta_{\{i_1, \ldots, i_j \} } v(\emptyset) \label{eq:mj}
\end{align}

Now consider a set $S$ of size $k$. Let $\pi S = \{i_1, i_2, \ldots, i_k \}$. W.l.o.g. assume $i_1 < i_2 <...< i_k$.
The set of predecessors of $i_1$ in this permutation are $\{1, \ldots, i_1 - 1 \}$ etc. In fact, $\pi^S = \{1, \ldots, i_1 - 1 \}$.


Define the following sets:
\begin{align}
&S^j := \{1, \ldots,j\} \text{~~for $j \geq 1$ ~~and~~} S^0 := \emptyset  \notag \\
\end{align}


Now consider the following sum over different choices of $i_1$:

\begin{align*}
\sum_{0 < j < i_2}    \interaction_{\{j, i_2, \ldots, i_k \}, \pi}(v) 
& = \sum_{0 < j < i_2} \delta_{\{j, i_2, \ldots, i_k \}} v(S^{j-1}) \\
& = \sum_{0 < j < i_2} \delta_{\{i_2, \ldots, i_k \}} v(S^{j}) - \delta_{\{i_2, \ldots, i_k \}} v(S^{j-1}) \\
& = \delta_{\{i_2, \ldots, i_k \}} v(\{1, \dots, i_2-1\}) - \delta_{\{i_2, \ldots, i_k \}} v(\emptyset) \\
\end{align*}

This gives us the following equation:
\begin{equation}\label{eq:telescope}
    \sum_{0 < j < i_2} \delta_{\{j, i_2, \ldots, i_k \}} v(S^{j-1}) = \delta_{\{i_2, \ldots, i_k \}} v(\{1, \dots, i_2-1\}) - \delta_{\{i_2, \ldots, i_k \}} v(\emptyset)
\end{equation}

\todo{The base case of what? also refer back to eq 17 below}

The base case is 
\begin{equation}\label{eq:telescopebase}
    \sum_{0 < j \leq n} \delta_{\{j\}} v(S^{j-1}) = v(N) - v(\emptyset)
\end{equation}

We repeatedly apply Equation~\ref{eq:telescope} and combine it with Equation~\ref{eq:telescopebase} for the base case to get
\begin{align*}
    \sum_{\{i_1 < \ldots < i_k \}} \delta_{\{i_1, i_2, \ldots, i_k \}} v(S^{i_1-1}) = v(N) - v(\emptyset) - \sum_{1 \leq j < k} M_j
\end{align*}

Since, $\delta_{\{i_1, i_2, \ldots, i_k \}} v(S^{i_1-1}) = \interaction_{S, \pi}(v)$, we can rewrite above as
$$
v(N) - v(\emptyset) = \sum_{1 \leq j < k} \sum_{|S| = j} \interaction_{S, \pi}(v)  + \sum_{|S| = k } \interaction_{S, \pi}(v)
$$
This shows the efficiency axiom for each permutation $\pi$. Since \prefixvalues are defined as expectation over all permutations, it is easy to see that \prefixvalues also satisfy the efficiency axiom.
\end{proof}


\subsubsection*{Proof of Proposition~\ref{prop:efficiency}}

We start by defining some notation.
\begin{align*}
M_j & :=  \sum_{|S| = j} \delta_{S} v(\emptyset) 
\end{align*}

First we prove a lemma connecting \prefixvalues of order $k$ and \prefixvalues of order $k-1$. An inductive application  of this lemma combined with the definition of $M_j$ gives the proof of proposition~\ref{prop:efficiency}.


\begin{lemma}\label{lemma:redistrib}
$$
\sum_{S, |S| = k} \mathcal{I}^{k}_{S, \pi}   = \sum_{S', |S'| = k-1} \mathcal{I}^{k-1}_{S', \pi} - M_{k-1}
$$
\end{lemma}
\begin{proof}
Notice that the right side of the question has only sets of size $k-1$. We first establish a connection between a set of size
$k-1$ and the sets of size $k$ (left side).

First we define some notation:
\begin{equation}
S^j := \{1, \ldots,j\} \text{~~for $j \geq 1$ ~~and~~} S^0 := \emptyset  \notag \\
\end{equation}


Consider the following sum over different choices for $i_1$:
\begin{align*}
    \sum_{0 < j < i_2} \delta_{\{j, i_2, \ldots, i_k \}} v(S^{j-1}) 
    & = \sum_{0 < j < i_2} \delta_{\{i_2, \ldots, i_k \}} (\delta_{\{j\}} v(S^{j-1}) \\
    & = \delta_{\{i_2, \ldots, i_k \}} (\sum_{0 < j < i_2} \delta_{\{j\}} v(S^{j-1})) \\
    & = \delta_{\{i_2, \ldots, i_k \}} (\sum_{0 < j < i_2} (v(S^{j}) - v(S^{j-1}))) \\
    & = \delta_{\{i_2, \ldots, i_k \}} (v(S^{i_2 - 1} - v(\emptyset)) \\
    & = \delta_{\{i_2, \ldots, i_k \}} v(S^{i_2 - 1} -  \delta_{\{i_2, \ldots, i_k \}} v(\emptyset)) \\    
\end{align*}
Thus we have the following relation that relates two derivatives for sets of size $k-1$ on the right side, with 
a sum over one element of order $k$ derivatives on the left side:
\begin{equation}
    \sum_{0 < j < i_2} \delta_{\{j, i_2, \ldots, i_k \}} v(S^{j-1}) = \delta_{\{i_2, \ldots, i_k \}} v(S^{i_2 - 1}) -  \delta_{\{i_2, \ldots, i_k \}} v(\emptyset)
\end{equation}

Next we sum this equation over all choices of $i_2 < \ldots < i_k$:

\begin{align*}
\sum_{S, |S| = k} \mathcal{I}^{k}_{S, \pi}(v)
& = \sum_{0 < i_1 < \ldots < i_k} \mathcal{I}^{k}_{S, \pi}(v) \\
& = \sum_{0 < i_1 < \ldots < i_k} \delta_{\{i_1, \ldots, i_k \}} v(S^{i_1-1})  \\
& = \sum_{0 < i_2 < \ldots < i_k} \sum_{0 < j < i_2} \delta_{\{j, i_2, \ldots, i_k \}} v(S^{j-1})  \\
& = \sum_{0 < i_2 < \ldots < i_k}  \delta_{\{i_2, \ldots, i_k \}} v(S^{i_2 - 1}) -  \delta_{\{i_2, \ldots, i_k \}} v(\emptyset) \\
& = \sum_{S', |S'| = k-1} \mathcal{I}^{k-1}_{S', \pi} - \sum_{|S'| = k-1} \delta_{S} v(\emptyset) \\ 
& = \sum_{S', |S'| = k-1} \mathcal{I}^{k-1}_{S', \pi} - M_{k-1} \\ 
\end{align*}

This finishes the proof of the Lemma.
\end{proof}

To finish the proof of Proposition~\ref{prop:efficiency}, we use induction. Lemma~\ref{lemma:redistrib} provides the inductive
step:
\begin{equation}\label{eq:inductive_step}
  \sum_{S', |S'| = k-1} \mathcal{I}^{k-1}_{S', \pi} =  M_{k-1} +  \sum_{S, |S| = k} \mathcal{I}^{k}_{S, \pi}
\end{equation}


The base case for induction is 
\begin{align*}
\sum_{S', |S'| = 1} \mathcal{I}^1_{S', \pi} & = \sum_{j} \delta_{\{j\}} v(S^{j-1}) \\
& = v(N) - v(\emptyset)
\end{align*}

Thus we have 
\begin{align*}
  v(N) - v(\emptyset) & = \sum_{j < k} M_j + \sum_{S, |S| = k} \mathcal{I}^{k}_{S, \pi}
\end{align*}

Taking expectation over all permutations, we get 

\begin{align*}
  v(N) - v(\emptyset) & = \sum_{j < k} M_j + \sum_{S, |S| = k} \mathcal{I}^{k}_{S} \\
  & = \sum_{j < k} \sum_{S', |S'| = j} \delta_{S'} v(\emptyset) + \sum_{S, |S| = k} \mathcal{I}^{k}_{S} \\
  & = \sum_{j < k} \sum_{S', |S'| = j} \interaction_{S'} + \sum_{S, |S| = k} \interaction_{S} \\
  & = \sum_{S, |S| \leq k} \interaction_{S} \\
\end{align*}
This concludes the proof of Proposition~\ref{prop:efficiency}.


Notice that Equation~\ref{eq:inductive_step} is very similar to the derivation of the Lagrange remainder term using integration by parts.\todo{Citation?}



\subsection{Connection to Taylor series}\label{sec:taylor}
In this section, we study multilinear extensions of games. We show a one-to-one correspondence between the terms in the Taylor series of the multilinear extension of a game and the \prefixvalues of the game.

\emph{Multilinear extension} of a game was first introduced by Owen~\cite{Owen72}. He showed that there is a unique multilinear function that coincides with $v$ on the corners of the cube $\{0, 1\}^N$. 
The multilinear extension of $v$ is defined as follows:

\begin{equation}\label{eq:multilinear}
f(x) = \sum_{S \subseteq N} \V(S) \prod_{i \in S} x_i \prod_{i \not\in S} (1 - x_i)     
\end{equation}

where $x_i \in [0, 1], i \in N$. The multilinear extension has a probabilistic interpretation: if player $i$ participates in the game with probability $x_i$, then $f(x)$ denotes the expected value of the game.

Owen~\cite{Owen72} showed the connection between Shapley values and the partial derivatives of $f$. In particular, integrating $f_j$ along the main diagonal of the cube gives Shapley value $\phi_j(v)$  (here $f(t) = f(t, t, \ldots, t)$ denotes the main diagonal of the cube, for $t \in [0, 1]$). 


Hammer and Rudeanu~\cite{Hammer68} showed that Equation~\ref{eq:multilinear} is equivalent to the following. We use this definition in our proofs below.
\begin{equation}\label{eq:altmultilinear}
f(x) = \sum_{T \subseteq N} a(T) \prod_{i \in T} x_i    
\end{equation}

We'll consider the unanimity games $u_T$ and the corresponding multilinear extension $f_T(x) = \prod_{i \in T} x_i$.
We prove the connection with Taylor series for the unanimity games; the general case follows from additivity.

We start with the $(k-1)^{\text{th}}$ order Taylor expansion with Lagrange remainder:

\begin{equation}\label{eq:taylor}
 f_T(1) - f_T(0) = \frac{f_T'(0)}{1 !} + \ldots +  \frac{f_T^{(k-1)}(0)}{(k-1)!} + \int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!} f_T^{(k)}(t) dt
\end{equation}

We show that the the terms on the right side of this equation correspond to the \prefixvalues for different sizes of sets.

First, we note that $f(1) = \V(N)$ and $f(0) = \V(\emptyset)$.

\begin{proposition}\label{prop:taylorterm}
Let $k$ be the order of explanation. The $j^{\text{th}}$ derivative of $f$ is the sum of interaction values over sets of size $j < k$.
$$\frac{f_T^{(j)}(0)}{j !} = \sum_{|S| = j} \interaction_{S}(v)$$
\end{proposition}
\begin{proof}

For a set $S \subseteq N$, $|S| = j$, define 
$$\Delta_S f_T(x) := \frac{\partial^{s} f_T}{\partial x_{i_1} \ldots \partial x_{i_j}} \text{~~~where~~} S = \{i_1, \ldots, i_j \}$$ 
Using Equation~\ref{eq:altmultilinear}, we get 
$$\Delta_S f_T(x) = \prod_{i \in T \setminus S} x_i \text{~~~if $S \subseteq T$}   $$
$1$ when $S = T$ and $0$ otherwise.
\todo{Use case statement.}

Hence $\Delta_S f_T(0) = 1$ iff $S = T$ and $0$ otherwise.

\begin{equation}\label{eq:taylorterm1}
\Delta_S f_T(0) = \interaction_S (u_T)    
\end{equation}


Now we evaluate $f_T^{(j)}(0)$:
\begin{align*}
\frac{f_T^{(j)}(0)}{j !} & = \frac{1}{j!} \sum_{i_1} \sum_{i_2} \cdots \sum_{i_j} \frac{\partial^{j} f_T (0)}{\partial x_{i_1} \ldots \partial x_{i_j}} \\
\end{align*}
Notice that $f_T$ is a multilinear function. Therefore, 
 only the mixed partial terms survive. Furthermore, all $j!$ mixed partials wrt $x_{i_1}, \ldots, x_{i_j}$ are identical. Hence, we can simplify the above equation to:

\begin{align*}
\frac{f_T^{(j)}(0)}{j !} & = \sum_{i_1 < i_2 < \ldots < i_j} \frac{\partial^{j} f_T (0)}{\partial x_{i_1} \ldots \partial x_{i_j}} \\
& = \sum_{S \subseteq N, |S| = j} \Delta_S f_T(0) \\
& = \sum_{S \subseteq N, |S| = j} \interaction_S(u_T) \\
\end{align*}

This proves the result.
\end{proof}

Next we analyze the Lagrange Remainder term in Equation~\ref{eq:taylor}. Next proposition establishes the connection to \prefixvalues.


\begin{proposition}\label{prop:lagrangeterm}
Let $k$ be the order of explanation for \prefixvalues. The Lagrange Remainder term is related to \prefixvalues as follows:
\begin{equation}
     \int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!} f_T^{(k)}(t) dt = \sum_{S \subseteq N, |S| = k} \interaction_{S}(u_T)
\end{equation}

\end{proposition}
\begin{proof}
As in the proof of Proposition~\ref{prop:taylorterm}, in the derivative of $f_T$, only the mixed partial terms are left:

\begin{align*}
\frac{f_T^{(k)}(t)}{k !} & = \sum_{S \subseteq N, |S| = k} \Delta_S f_T(t) & \\
\end{align*}

We use this expression in Lagrange remainder term and interchanging the order of integral and summation. Note that there is an extra factor of $k$ that survives on the right side.
\begin{align}\label{eq:lagrangesum}
\int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!}  f_T^{(k)}(t) dt   
& = \sum_{S \subseteq N, |S| = k}  \int_{t=0}^1 k (1-t)^{k-1} \Delta_S f_T(t) dt
\end{align}
We evaluate the term inside the summation and show that it is indeed $\interaction_S(u_T)$. We use Eqaution~\ref{eq:altmultilinear} to evaluate $\Delta_S f(t)$:

\begin{align}
\int_{t=0}^1 k (1-t)^{k-1} \Delta_S f_T(x) dx
& = \int_{x=0}^1 k (1-x)^{k-1}  \left( \prod_{i \in T \setminus S} x \right) dx & \text{(it's $0$ if $S \not\subseteq T$} \notag \\
& = \int_{t=0}^1 k (1-t)^{k-1}  \left(x^{t-k} \right) dt & \text{$|T| = t$ and $|S| = k$} \notag \\
& =  k \int_{t=0}^1 t^{t-k} (1-t)^{k-1} dt & \notag \\
& = k \cdot B(u+1, k) & \text{$B(\cdot, \cdot)$ is the Beta function}\notag \\
& = 1 / {t \choose k}
& = \interaction_S(u_T) & \text{from Equation~\ref{eq:unanimity_stv}}\label{eq:lagrange_inter}
\end{align}

Along with Equation~\ref{eq:lagrangesum}, this gives us
\begin{equation*}
    \frac{1}{k!} \int_{t=0}^1 (1-t)^{k-1} f_T^{(k)}(t) dt = \sum_{S \subseteq N, |S| = k} \interaction_{S}(v)
\end{equation*}
This finishes the proof.
\end{proof}


\subsection{Connection to Taylor series}\label{sec:taylor}
In this section, we connect \stv to the Taylor series.

%We show a one-to-one correspondence between the terms in the Taylor series of the multilinear extension of a \game and the \stv of the \game.

%\emph{Multilinear extension} of a \game was first introduced by Owen~\cite{Owen72}. He showed that there is a unique multilinear function that coincides with $v$ on the corners of the cube $\{0, 1\}^N$. 
The multilinear extension of $\V$ is defined as follows:

\begin{equation}\label{eq:multilinear}
f(x) = \sum_{S \subseteq N} \V(S) \prod_{i \in S} x_i \prod_{i \not\in S} (1 - x_i)     
\end{equation}

where $x_i \in [0, 1], i \in N$. The multilinear extension has a probabilistic interpretation: if \player $i$ set with probability $x_i$, then $f(x)$ denotes the expected value of the \game. Consider the line from $\emptyset$ to $N$: $f(t, \ldots, t)$ for $t \in [0, 1]$ (we'll denote it as $f(t)$ in shorthand). For a set $S \subseteq N$, with $|S| = j$, define 
$$\Delta_S f(x) := \frac{\partial^{j} f}{\partial x_{i_1} \ldots \partial x_{i_j}} \text{~~~where~~} S = \{i_1, \ldots, i_j \}$$
Consider the $(k-1)^{\text{th}}$ order Taylor expansion of $f(\cdot)$ at $0$ with Lagrange remainder of the function $f$ and consider the multivariate expansion of each term:
\begin{align}\label{eq:taylor}
 f(1) - f(0) & = \frac{f'(0)}{1 !} + \ldots +  \frac{f^{(k-1)}(0)}{(k-1)!} + \int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!} f^{(k)}(t)  dt \\
 & = \sum_{1 \leq j \leq k-1} \sum_{S \subseteq N, |S| = j} \Delta_S f(0) + \sum_{S \subseteq N, |S| = k} \int_{t=0}^1 k (1-t)^{k-1} \Delta_S f(t) dt
\end{align}

\begin{theorem}
\label{thm:taylorterm}
Let $k$ be the order of explanation and $j < k$. Then $j^{\text{th}}$ order \stv can be obtained from the $j^{\text{th}}$ order terms in the Taylor series. 
$$\Delta_S f(0) = \interaction_{S}(\V) \text{~~~where~~} |S| < k$$ 
The $k^{\text{th}}$ order \stv can be obtained from the Lagrange remainder term of the Taylor series:
$$ int_{t=0}^1 k (1-t)^{k-1} \Delta_S f(t) dt = \interaction_{S}(\V) \text{~~~where~~} |S| = k$$
\end{theorem}
We give the proof of this theorem in the appendix.


\cite{Owen72} showed that integrating $f_j$ along the main diagonal of the cube gives Shapley value $\phi_j(v)$  (here $f(t) = f(t, t, \ldots, t)$ denotes the main diagonal of the cube, for $t \in [0, 1]$). 








We'll consider the unanimity \games $u_T$ and the corresponding multilinear extension:
\begin{equation}\label{eq:unanimity-multilinear}
f_T(x) = \prod_{i \in T} x_i     
\end{equation}

We prove the connection with Taylor series for the unanimity \games. Since unanimity \games form the basis, the general case follows from linearity axiom. We start with the $(k-1)^{\text{th}}$ order Taylor expansion with Lagrange remainder:

\begin{equation}\label{eq:taylor}
 f_T(1) - f_T(0) = \frac{f_T'(0)}{1 !} + \ldots +  \frac{f_T^{(k-1)}(0)}{(k-1)!} + \int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!} f_T^{(k)}(t) dt
\end{equation}

We show that the the terms on the right side of this equation correspond to the \stv for different sizes of sets.

First, we note that $f(1) = \V(N)$ and $f(0) = \V(\emptyset)$.

\begin{proposition}\label{prop:taylorterm}
Let $k$ be the order of explanation. The $j^{\text{th}}$ derivative of $f$ is the sum of interaction values over sets of size $j < k$.
$$\frac{f_T^{(j)}(0)}{j !} = \sum_{|S| = j} \interaction_{S}(\V)$$
\end{proposition}
\begin{proof}

For a set $S \subseteq N$, $|S| = j$, define 
$$\Delta_S f_T(x) := \frac{\partial^{s} f_T}{\partial x_{i_1} \ldots \partial x_{i_j}} \text{~~~where~~} S = \{i_1, \ldots, i_j \}$$ 
Using Equation~\ref{eq:unanimity-multilinear}, we get 
\begin{align*}
\Delta_S f_T(x) & = \prod_{i \in T \setminus S} x_i \text{~~~iff $S \subseteq T$}     \\
& = 1 \text{when $S = T$ and $0$ otherwise.}
\end{align*}
Hence $\Delta_S f_T(0) = 1$ iff $S = T$ and $0$ otherwise. This gives us:
\begin{equation}\label{eq:taylorterm1}
\Delta_S f_T(0) = \interaction_S (u_T)    
\end{equation}

Now we evaluate $f_T^{(j)}(0)$:
\begin{align*}
\frac{f_T^{(j)}(0)}{j !} & = \frac{1}{j!} \sum_{i_1} \sum_{i_2} \cdots \sum_{i_j} \frac{\partial^{j} f_T (0)}{\partial x_{i_1} \ldots \partial x_{i_j}} \\
\end{align*}
Notice that $f_T$ is a multilinear function. Therefore, 
 only the mixed partial terms survive. Furthermore, all $j!$ mixed partials wrt $x_{i_1}, \ldots, x_{i_j}$ are identical. Hence, we can simplify the above equation to:

\begin{align*}
\frac{f_T^{(j)}(0)}{j !} & = \sum_{i_1 < i_2 < \ldots < i_j} \frac{\partial^{j} f_T (0)}{\partial x_{i_1} \ldots \partial x_{i_j}} \\
& = \sum_{S \subseteq N, |S| = j} \Delta_S f_T(0) \\
& = \sum_{S \subseteq N, |S| = j} \interaction_S(u_T) \\
\end{align*}

This proves the result.
\end{proof}

Next we analyze the Lagrange Remainder term in Equation~\ref{eq:taylor}. Next proposition establishes the connection to \stv.

\begin{proposition}\label{prop:lagrangeterm}
Let $k$ be the order of explanation for \stv. The Lagrange Remainder term is related to \stv as follows:
\begin{equation}
     \int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!} f_T^{(k)}(t) dt = \sum_{S \subseteq N, |S| = k} \interaction_{S}(u_T)
\end{equation}

\end{proposition}
\begin{proof}
As in the proof of Proposition~\ref{prop:taylorterm}, in the derivative of $f_T$, only the mixed partial terms are left:

\begin{equation*}
\frac{f_T^{(k)}(t)}{k !} = \sum_{S \subseteq N, |S| = k} \Delta_S f_T(t) 
\end{equation*}

We use this expression in Lagrange remainder term and interchanging the order of integral and summation. Note that there is an extra factor of $k$ that survives on the right side.
\begin{align}\label{eq:lagrangesum}
\int_{t=0}^1 \frac{(1-t)^{k-1}}{(k-1)!}  f_T^{(k)}(t) dt   
& = \sum_{S \subseteq N, |S| = k}  \int_{t=0}^1 k (1-t)^{k-1} \Delta_S f_T(t) dt
\end{align}
We evaluate the term inside the summation and show that it is indeed $\interaction_S(u_T)$. We use Eqaution~\ref{eq:unanimity-multilinear} to evaluate $\Delta_S f(t)$:

\begin{align}
\int_{t=0}^1 k (1-t)^{k-1} \Delta_S f_T(x) dx
& = \int_{x=0}^1 k (1-x)^{k-1}  \left( \prod_{i \in T \setminus S} x \right) dx & \text{(it's $0$ if $S \not\subseteq T$} \notag \\
& = \int_{t=0}^1 k (1-t)^{k-1}  \left(x^{t-k} \right) dt & \text{$|T| = t$ and $|S| = k$} \notag \\
& =  k \int_{t=0}^1 t^{t-k} (1-t)^{k-1} dt & \notag \\
& = k \cdot B(u+1, k) & \text{$B(\cdot, \cdot)$ is the Beta function}\notag \\
& = 1 / {t \choose k} ~ ~ ~ = \interaction_S(u_T) & \text{from Equation~\ref{eq:unanimity_stv}}\label{eq:lagrange_inter}
\end{align}

Along with Equation~\ref{eq:lagrangesum}, this gives us
\begin{equation*}
    \frac{1}{k!} \int_{t=0}^1 (1-t)^{k-1} f_T^{(k)}(t) dt = \sum_{S \subseteq N, |S| = k} \interaction_{S}(v)
\end{equation*}
This finishes the proof.
\end{proof}


As we have seen in Propositions~\ref{prop:taylorterm} and~\ref{prop:lagrangeterm}, each of the \stv
$\interaction_S(v)$ is related to $\Delta_S f(x)$. 
For $|S| < k$, it is $\Delta_S f(0)$. For $|S| = k$, it is $\int_{t=0}^1 k (1-t)^{k-1} \Delta_S f(t) dt$
(Equations~\ref{eq:taylorterm1} and~\ref{eq:lagrange_inter}). 

If we consider the case where $k = 1$, we see that the definition of \stv in Equation~\ref{eq:permutation} is exactly
the Shapley value. Furthermore, Proposition~\ref{prop:lagrangeterm} reduces to the result by \cite{Owen72} (Theorem~5).
Thus the \stv are a strict generalization of the Shapley values.



\subsection{Majority Function}

The majority \game $\V_{maj}$ over the set of \players $N$ is defined by $\V_{maj}(S) = 1$ if $|S| \geq n/2$ and is $0$ otherwise; here $n=|N|$.

It is easy to check that the singleton terms for pairwise \stv for a majority \games are uniformly zero (for $n >2$). The
pairwise terms are each equal to reciprocal of the number of pairs, $2/(n*(n-1))$, a simple consequence of symmetry and
efficiency. The analytical conclusion from this is that majority \games are all about interaction, and this is intuitively reasonable.

In contrast, the pairwise \siv are uniformly zero for every pair of \players (we exclude the calculation). This is unexpected; one would imagine that in a three \player majority \game there would be non-zero interaction values for sets of size $2$, the size at which majority arises. The results from studying pairwise \siv seems to suggest that there is \emph{no} pairwise interaction! However, \siv of larger interaction sizes do have non-zero values. For instance, for a majority \game with $3$ \players, the interaction value corresponding to all three \players is $-2$, a quantity that has no simple justification in itself. The pattern becomes even more confusing for majority \games of more \players.

Figure~\ref{fig:majority} shows the sum of the \siv (in log scale) for all subsets of \players for majority \games as number of \players increases. This displays two non-intuitive characteristics. First, the total interaction diverges (recall the plot is in log scale) despite the fact that the \game value being shared among the \players is constant ($1$). Second, the \emph{sign} of the total interaction alternates. In fact, for a \game of a fixed size, \emph{every} non-singleton interaction value has the same sign. (So the sign alternation is not due to cancellation across the interactions.) There is no intuitive reason for this sign alternation. 

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{siv_majority.png}
\caption{The sum of \siv (in log scale) for all subsets of \players for majority \games as a function of the number of \players.}
\label{fig:majority}
\end{figure}

This discussion highlights the value of the \stv interaction distribution approach over that of \siv. To study interactions using \siv, one has to compare $2^n$ quantities, and even then the results appear unstable. In contrast, studying $O(n^2)$ quantities using the pairwise \stv gives us some insight, no matter what the size of the set of interacting elements.






==> general_case.tex <==
\section{General case}

\subsection{Description of the method}

\subsection{\prefixvalues satisfy axioms}

    \item \emph{Dummy axiom} Straightforward.
    \item \emph{Linearity axiom} Expectation is linear.
    \item \emph{Symmetry axiom} The expectation is symmetric and taken over all permutations.
    \item \emph{Interaction distribution axiom} Consider an interaction game $v_T$ and $S$ such that $|S| < |T|$. Notice that $\interaction_S(v_T) = \delta_S(v_T) = \sum_{W \subseteq S} (-1)^{w-s} v_T(W)$. Since $|W| < |T|$, we know that each $v_T(W) = 0$. Hence $\interaction_S(v_T) = 0$.
    \item \emph{Efficiency} 
    
\begin{proposition}
\stv satisfy the efficiency axiom. Formally
$$\sum_{S, |S| \leq k} \interaction_{S}(v) = v(N) - v(\emptyset)
$$
\end{proposition}
\begin{proof}
%Consider a permutation $\pi$ and consider $\interaction_{S, \pi}(v)$ defined by Equation~\ref{eq:perminteraction}, where $|S| %= k$. We will show that $\interaction_{S, \pi}(v)$ satisfy efficiency. 

%Let $\{i_1, i_2, \ldots, i_k \}$ be the image of $S$ under the permutation $\pi$. W.l.o.g. assume $i_1 < i_2 <...< i_k$.

%\begin{equation*}
%\delta_\phi(T) := v(T)
%\end{equation*}

%For $T \subseteq N \setminus S$, we have
%\begin{equation}
%\delta_{i_1, i_2,...i_k}(T) := \delta_{i_2,...i_k}(T \cup \{i_1\}) - \delta_{i_2,...i_k}(T)  \text{~~~~ for $(k > 0)$}
%\end{equation}

\todo{kedar: make sure the notation matches.}
W.l.o.g. assume $i_1 < i_2 <...< i_k$.

\begin{equation}
\delta_\phi(S) := v(S) \notag
\end{equation}

\begin{equation}
\delta_{i_1, i_2,...i_k}(S) := \delta_{i_2,...i_k}(S \cup \{i_1\}) - \delta_{i_2,...i_k}(S) (k > 0) 
\end{equation}

\begin{equation}
I_{i_1, i_2,...i_k}^\pi(v) := \delta_{i_1, i_2,...i_k}(S)
\end{equation}
where $S = \pi^{i_1-1}$ if $i_1 > 0$ else $\phi$.


\begin{align}
&S^j := \{0, 1, ...,j\} (j >= 0),  \notag \\
&S^{-1} := \phi
\end{align}

\begin{equation}
M_k := \sum_{0 <= i_1 < i_2 < ... <i_k < n} \delta_{i_1,...i_k}(\phi)
\end{equation}

For $k >1$,
\begin{align}
&\sum_{0 <= j < i_2} I_{j, i_2,...i_k}^\pi(v) \notag\\
&= \sum_{0 <= j < i_2} \delta_{i_2,...i_k}(S^{j}) -  \delta_{i_2,...i_k}(S^{j-1}) \notag\\
&= \delta_{i_2,...i_k}(S^{i_2-1}) -  \delta_{i_2,...i_k}(\phi) \notag\\
&= I_{i_2, i_3,....i_k}^\pi(v) - \delta_{i_2,...i_k}(\phi) 
\end{align}

Note, for $k=1$,  
\begin{equation}
\sum_{0 <= j < n} I_{j}^\pi(v) = v(S) - v(\phi)
\end{equation}

Using the above, we can show
\begin{align}
&\sum_{0 <= i_1 < i_2 < ... <i_k < n} I_{i_1, i_2,...i_k}^\pi(v) \notag \\
&= v(S) - v(\phi) - \sum_{0<j<k} M_j
\end{align}




\end{proof}

    

\subsection{Uniqueness}
To prove uniqueness, we have to prove that any interaction index that satisfies axioms 1-5 matches \prefixvalues on unanimity games. Since unanimity games form a basis, the uniqueness follows.


\subsubsection{\prefixvalues on unanimity games}
Consider the unanimity game $u_T$ defined as $u_T(S) = 1$ if $T \subseteq S$, otherwise $0$. Fix $k$ to be the order of approximation for \prefixvalues. Let's consider $\interaction_S(u_T)$. We first prove a lemma about $\delta_S u_T$.

\begin{lemma}\label{lemma:dummydelta}
Discrete derivatives of unanimity games. For $T$ such that $S \not\subseteq T$
$\delta_S u_T(W) = 0$
\end{lemma}

\begin{proof}
$S \not\subseteq T$ implies that $S \setminus T \neq \emptyset$. Consider $i \in S \setminus T$. We have
$$\delta_S u_T(W) = \delta_{S \setminus i} (\delta_i u_T(W))$$.
Note that $\delta_i u_T(W) =  u_T(W \cup i) - u_T(W) = 0$, since $i \not\in T$.
Hence $\delta_S u_T(W) = 0$.
\end{proof}


We divide this into three cases:
\begin{enumerate}
    \item $|S| < k$: In this case, $\interaction_S(u_T)$ is defined as $\delta_S u_T(\emptyset)$. We compute this as:
    \begin{align*}
        \delta_S u_T(\emptyset) & = \sum_{W \subseteq S} (-1)^{w-s} u_T(W) \\
        & = \sum_{W \subseteq S, W \supseteq T} (-1)^{w-s}
    \end{align*}
    Note that this sum is $0$ if $T \not\subseteq S$. When $T \subset S$, we substitute $U = W \setminus T$
    \begin{align*}
        \delta_S(u_T, \emptyset) & = (-1)^{s-t} \sum_{U \subseteq S \setminus T} (-1)^{u} \\
        & = 0 \\
    \end{align*}
    
    Finally, for $S = T$, $\interaction_T(u_T) = \delta_T(u_T, \emptyset) = 1$.
    
    Thus, for $|S| < k$, we have $\interaction_S(v_T) = 1$ if $S = T$ and $0$ otherwise.
    
    \item $|S| = k$: this is \emph{remainder} term. 
    
    For a fixed permutation $\pi$, we have $\interaction_{S, \pi}(u_T) = \delta_{S} u_T(\pi^S)$, where $\pi^S = \cap_{i \in S} \pi^i$.
    
    Applying Lemma~\ref{lemma:dummydelta}, we know that, if $S \not\subseteq T$, then $\interaction_{S, \pi}(u_T) = 0$. Consequently, $\interaction_{S}(u_T)$ is zero. If $|T| < k$, it follows that $\interaction_{S}(u_T) = 0$.
    Finally, consider $T$ such that $S \subseteq T$. Let $S' \subseteq T$ such that $|S| = |S'|$. Let $\pi$ be a permutation of $N$ such that $\pi T = T$ and $\pi S = S'$. Then by the symmetry axiom, $\interaction_S(u_T) = \interaction_{\pi S}(\pi u_T) = \interaction_{S'}(u_{\pi T}) = \interaction_{S'}(u_T)$.
    
    Hence for each subset $S$ of $T$ with size $k$, the interaction term is identical. Using completeness axiom,
    $$ \sum_{S \subseteq T, |S| = k} \interaction_{S}(u_T)  = 1$$
    Hence each must be equal to $\frac{1}{{t \choose k}}$

    
\end{enumerate}

\subsubsection*{Finishing proof of uniqueness}

Consider a unanimity game $u_T$ and an interaction index $\phi_S$ that satisfies axioms 1-5.
We want to derive $\phi_S(u_T)$ using the axioms.

Start with dummy axiom. If $i \not\in T$, then $i$ is a dummy player for $u_T$. This implies that if $S \setminus T \neq \emptyset$, then $\phi_S(u_T) = 0$.

Consider $|S| < k$. Interaction distribution axiom states that $\phi_S(u_T) = 0$ if $|S| < |T|$. Next we use the dummy axiom. Note that, for all $j \not\in T$, $\delta_j(u_T) = 0$. Thus $j$ is dummy player. Dummy axiom implies that $\phi_S(u_T) = 0$ if $j \in S$. Hence, $\phi_S(u_T) = 0$ for all $S$ such that $|S \setminus T| > 0$.

Using efficiency axiom, we have $\sum_S \phi_S(u_T) = u_T(N) = 1$. As we saw before, $\phi_S(u_T) = 0$ if $S \neq T$.
Hence the sum reduces to  $\phi_S(u_S) = 1$, when $S = T$.

Finally, consider the case where size of $S$ is same as the order of explanation, i.e.  $|S| = k$.
As we saw earlier, $\phi_S(u_T) = 0$ if $S \not\subseteq T$. Using efficiency axiom:
$\sum_{S \subseteq T}  \phi_{S}(u_T)  = 1$. Furthermore, since $k$ is the order of explanation, the interaction index is
defined to be $0$ for sets larger than $k$. Hence, $\sum_{S \subseteq T, |S| = k}  \phi_{S}(u_T)  = 1$.

Symmetry axiom implies that each of these terms must be equal. Hence $\phi_{S}(u_T) = $\frac{1}{{t \choose k}}$.

This shows that any interaction index that satisfies axioms 1-5 matches the \prefixvalues on unanimity games. 
This proves the uniqueness for \prefixvalues.


\section{Generalization of \prefixvalues expression to k}

\begin{lemma}\label{lemma:mobius}
Mobius coefficients and discrete derivatives are related by following relation:
$$a(T \cup S) = \sum_{W \subseteq T} (-1)^{t-w} \delta_S v(W)$$
for $S$ and $T$ such that $S \cap T = \emptyset$.
\end{lemma}

\begin{proof}
$$a(T) = \sum_{W \subseteq T} (-1)^{t-s} v(W)$$
Let $S$ and $T$ be two sets such that $S \cap T = \emptyset$. We have
\begin{align*}
    a(T \cup S) 
& = \sum_{W' \subseteq T \cup S} (-1)^{t+s-w'} v(W') & \\
& = \sum_{W \subseteq T} \sum_{U \subseteq S} (-1)^{t+s-w-u} v(U \cup W) & \text{writing $W = W' \cap T$ and $U = W' \cap S$} \\
& = \sum_{W \subseteq T} (-1)^{t-w} \sum_{U \subseteq S} (-1)^{s-u} v(U \cup W) & \\
& = \sum_{W \subseteq T} (-1)^{t-w} \delta_S v(W) \\
\end{align*}
\end{proof}

\begin{proposition}
\prefixvalues satisfy the following expression:
$$ \interaction_{S}(v) = \frac{k}{n} \sum_{T \subseteq N \setminus S} \delta_S v(T)  \frac{1}{{n-1 \choose t}}$$
\end{proposition}

\begin{proof}
Consider a set $T$ such that $|T| > 1$. 

Let $a(T)$ be the \emph{M\"obius transform} defined as:
$$a(T) = \sum_{S \subseteq T} (-1)^{t-s} v(S), ~~~~~~ T \subseteq N$$

Decomposition of any function $v$ into unanimity games can be written in terms of $a(T)$'s as follows:
$$ v(S) = \sum_{T \subseteq N} a(T) u_T(S) $$

Using the linearity axiom, we can extend $\interaction_S$ from unanimity games to $v$ as follows:

\begin{align*}
 \interaction_{S}(v) & = \sum_{T \subseteq N} a(T) \interaction_{S}(u_T)  & \\
 & = \sum_{T \subseteq N, S \subseteq T} a(T) \frac{1}{t \choose k} & \text{$|S| = k$, the order of explanation} \\
 & = \sum_{W \subseteq N \setminus S} a(W \cup S) \frac{1}{w+k \choose k}  & \text{by setting $W = T \setminus S$} \\
 & = \sum_{W \subseteq N \setminus S}  \sum_{U \subseteq W} (-1)^{u-w} \delta_S v(U)  \frac{1}{w+k \choose k}  & \text{use Lemma~\ref{lemma:mobius}} \\ 

 & = \sum_{U \subseteq N \setminus S} \delta_S v(U) \sum_{W \supseteq U, W \subseteq N \setminus S} \frac{(-1)^{u-w}}{{w+k \choose k}}  & \text{exchanging summation} \\
\end{align*}

Now we analyze the inner sum. We use the following identity: ${w+k \choose k} = 1/(k \cdot B(w+1, k))$, where $B()$ is the Beta function.

\begin{align*}
 \sum_{W \supseteq U, W \subseteq N \setminus S} \frac{(-1)^{u-w}}{{w+k \choose k}} 
& =  \sum_{W \supseteq U, W \subseteq N \setminus S} (-1)^{u-w} k \cdot B(w+1, k) & \\
& = k \sum_{w=u}^{n-k} {n-k-u \choose w-u} (-1)^{u-w} B(w+1, k) & \\
& = k \sum_{w=u}^{n-k} {n-k-u \choose w-u} (-1)^{u-w} \int_{0}^1 x^w (1-x)^{k-1} dx & \\
& = k \int_{0}^1 \sum_{w=u}^{n-k} {n-k-u \choose w-u} (-1)^{u-w} x^w (1-x)^{k-1} dx & \text{exchange sum \& integral} \\
& = k \int_{0}^1 x^u (1-x)^{k-1} \sum_{w'}^{n-k-u} {n-k-u \choose w'} (-1)^{w'} x^{w'} dx & \text{setting $w' = w-u$} \\
& = k \int_{0}^1 x^u (1-x)^{k-1} (1-x)^{n-k-u} & \\
& = k B(u+1, n-u) & \text{using Beta function} \\
& = \frac{k}{n} \frac{1}{{n-1 \choose u}}
\end{align*}

We use this expression for the inner sum in the above equation to get:
$$\interaction_{S}(v) = \frac{k}{n} \sum_{U \subseteq N \setminus S} \delta_S v(U)  \frac{1}{{n-1 \choose u}} $$
This finishes the proof.
\end{proof}



==> response.tex <==
%----------------------------------------------------------------------------------------------------------------------

\newpage
\nolinenumbers
\pagenumbering{gobble}

\subsubsection*{Response to reviewers}
We thank the reviewers for their comments and questions. We have addressed these below.

\paragraph{Novelty of the work} Reviewer 2  says "Novelty of the axiomatic definitions is limited by the fact that much of it has been published before.
"

The Shapley Taylor value, our key idea, has never been published before. It involves a novel axiom (the interaction distribution axiom),
and a new axiomatic result (Theorem 2). 
(It is the only published interaction detection method that provably satisfies the efficiency axiom, which allows us to aggregate attributions (as in the feature selection task below), and compare interaction effects with singleton effects (cf. Figure 1). Other methods can have attribution magnitudes that are not commensurate with the prediction score (cf. Sections 4.1 and 4.2).)

The connection between the Taylor series and the attribution problem is also new. In contrast, most of the other "axiomatic" work simply applies prior results from cooperative game theory.  This is \emph{primarily a theory paper}, and we hope it is judged on the merit of its novel theoretical contributions. 

\paragraph{Importance of the work}
 Reviewer 1 asks about robustness of the measure to poor model fit. Separately,  Reviewers 1 and 2 asked about the gain from studying feature interactions.
 
 In our mind the main gain is to aid model validation. Attributions/Local Feature importance have had successful application in validating models. For some models, base feature importance is not directly indicative of validity. We expect our work to be helpful here. For instance,
 
 \begin{enumerate}
 \item In a sentiment detection model, we expect an interaction between modifiers and  sentiment bearing terms. Modifiers could be negation (good vs. not good), intensifiers (bad vs. very bad) etc. Table 1 gives several examples of these types of interactions. Here are some more examples of incorrect interactions:
 \begin{itemize}
     \item In the sentence: "García Bernal and Talancón are an \textbf{immensely} appealing couple , and even though their story is \textbf{predictable} , you 'll want things to work out ." there is a large negative interaction (of score $-0.32$) between 'immensely' and 'predictable'. This is incorrect because in the sentence construction, 'immensely' does not modify 'predictable'.
     \item In the sentence: "It 's \textbf{not} life-affirming -- its \textbf{vulgar} and mean , but I liked it", there is a negative interaction between positive interaction between 'not' and 'vulgar' despite the fact that not does not modify vulgar.
 \end{itemize}
 
 
 \item In question answering tasks, we would expect words from the question to match words from the text (Figure 3 shows examples of this.)
 
 \item In recommender systems, user features have to match document (music/video) features. 
 \end{enumerate}
 
 In all of these examples, attributions do not result in validation, and studying interaction is a must.
 
 Reviewer 1 hints at using our technique for feature selection, and comparing with ANOVA. Unlike our method, ANOVA typically works across the entire data set, not a specific input. We did not set out to study such "global" feature importance. However, prompted by the reviews, we did a small experiment that indicates that this is an interesting future direction, though we certainly cannot claim any success yet.
 We applied our method for feature selection on the well-known Boston housing dataset, and compared it to Lasso, arguably the foremost feature selection method.
 
 Here are some details.  This dataset has 13 features. We trained a random forest model on the dataset and use Shapley-Taylor values aggregated across training data to identify important feature crosses (out of 78 possible crosses).
 (Notice that this aggregation is only meaingful because of the "efficiency" axiom---because the attributions are in the units of the predictions, we can aggregate them.)
 
 
 We use these importance scores to do feature selection over
singleton and crossed features.
We compare it to feature selection based on Lasso, where the set of features available to Lasso is singleton features and crosses. In both cases, we apply linear regression over the selected features. We show the mean-squared error on test set for the two methods of feature selection in the figure below.

\begin{figure}[!h]
  \includegraphics[width=0.6\linewidth]{lasso_vs_stv2.png}
  \caption{{\small Comparison of feature cross selection. X-axis shows number of features (singletons or crosses) selected. Y-axis shows Mean Squared Error for two feature selection methods.}}
    \label{fig:lasso_vs_stv}
  \end{figure}


It appears that on this limited test, \stv values are comparable if not better than Lasso. 

\paragraph{Computation efficiency} Reviewer 3 says 
"authors do not discuss computational aspects of their model explanations."

We accept that we did not do this in detail, and will elaborate how we achieved computational efficiency: 

\begin{enumerate}

\item We restricted application of \stv values only to important features that we identified using an attribution technique called Integrated Gradients.

\item Sampling techniques have been applied to Shapley computation (\emph{Bounding the Estimation Error of Sampling-based Shapley Value Approximation} by 
Sasan Maleki, Long Tran-Thanh, Greg Hines, Talal Rahwan and Alex Rogers), which improves the computational efficiency of the Shapley value by sampling permutations. For \stv, by replacing the expectation in our Equation 5 by an average over sample random permutations). The analysis technique of Maleki et al also applies for \stv. In particular, we can prove that  if the number of samples $m \geq \lceil \frac{2 \ln(2/\delta) r^2}{\epsilon^2} \rceil $, then for a fixed pair of features $(i, j)$, we have $\mathrm{Pr}(|\hat{\phi_{ij}} - \phi_{ij}| > \epsilon) < \delta$.

\item Reviewer 3 additionally pointed us to the L-Shapley method that relies on locality of interaction structure to get a
fast approximation of Shapley values. This is a very interesting work. We think that our Theorem 1 can be used in a similar
way to get a fast approximation. We leave this as future work.
\end{enumerate}



\paragraph{Rigorous presentation} Reviewer 2 raised a question around representation of set vs vectors. We'll make this more rigorous in the paper. (The correspondence between the binary vector of length $n$ and a set $S$ is 
simply that $i^{th}$ entry of the vector is $1$ iff $i \in S$. ``Removing'' a feature from the input set means setting the feature to the baseline feature value. Thus, the vector $(1, 1, \ldots, 1)$ (all ones) corresponds to the input
instance under consideration, while the vector $(0, 0, \ldots, 0)$ (all zeros) corresponds to setting all the features to their baseline values. As a concrete example, for the question answering model, removing a word from a question is done by replacing it with <PAD> token.)

\paragraph{Comparison with other methods} Reviewers 1 and 2 have asked about comparison to other methods.
Most of the related work (Section 1.2.2) on feature interactions is about studying global interactions. The only exception is Shapley interaction values, which we do compare with.



\paragraph{Related work} Reviewer 3 has pointed out a few related papers. We thank the reviewer for bringing these to our notice. We will include these in our related work section.



% ID:  50 -->  García Bernal and Talancón are an immensely appealing couple , and even though their story is predictable , you 'll want things to work out .
% immensely (0.475) x predictable (-0.878): -0.327 (frac: 0.557)

%ID:  69 -->  For devotees of French cinema , Safe Conduct is so rich with period minutiae it 's like dying and going to celluloid heaven .
% Safe (1.674) x heaven (1.550): -0.458 (frac: -0.310)
